Multi-Channel Stochastic Variational Inference for the Joint Analysis of Heterogeneous Biomedical Data in Alzheimer's Disease

The joint analysis of biomedical data in Alzheimer's Disease (AD) is important for better clinical diagnosis and to understand the relationship between biomarkers. However, jointly accounting for heterogeneous measures poses important challenges related to the modeling of the variability and the interpretability of the results. These issues are here addressed by proposing a novel multi-channel stochastic generative model. We assume that a latent variable generates the data observed through different channels (e.g., clinical scores, imaging, ...) and describe an efficient way to estimate jointly the distribution of both latent variable and data generative process. Experiments on synthetic data show that the multi-channel formulation allows superior data reconstruction as opposed to the single channel one. Moreover, the derived lower bound of the model evidence represents a promising model selection criterion. Experiments on AD data show that the model parameters can be used for unsupervised patient stratification and for the joint interpretation of the heterogeneous observations. Because of its general and flexible formulation, we believe that the proposed method can find important applications as a general data fusion technique.

==> tex/Discussion.tex <==
\section{Discussion}

\ldots \\
The lower bound is a good approximation of the marginal likelihood, which provides a basis for selecting a model [\figref{fig:model_sel_lin}]
Though this may work in practice, model selection based on the lower bound is not justified in theory [\cite{Blei2016}].
\ldots

% Efficient prediction $\p{\x_i|\x_{c \neq i}}$ can be made for every channel given When only data from a single channel is provided \ldots \\
% 
% Being a parametric method, trining dataset doesn't need to be all stored in memory.
% 
% Allow any combination of channels to be present or absent at test time without the need to train an exponential number of models \cite{Ngiam2011} \\
% 
% In \cite{Amin2016} is not clear if it's extensible to multiple views/channels 
% 
% Var Inference not always good \cite{Yao2018} \\
% 
% In many applications, we have access to multiple views of data at training time while only one view is available at test time. \\
% 
% \section{extension}
%  The main challenge with the healthcare data comes from genetics and imaging, that are high-dimensional (thousands of genes; million of voxels) and complex (gene interactions; multi-modal imaging).
% Moreover, capturing the patient’s behavioral data through several sensors and combining them with standard clinical data adds additional layers of complexity.


==> tex/Notes.tex <==
\section{Notes}
\begin{equation}
\begin{aligned}
&\p{\z|\setx} \\
&\p{z|\x_1} \longmapsto \text{}  q{z|\phib_1, \x_1}\\
&\p{z|\x_C} \\
\end{aligned}
\end{equation}

